Semi-supervised Quality Evaluation of Colonoscopy Procedures

Colonoscopy is the standard of care technique for detecting and removing polyps for the prevention of colorectal cancer. Nevertheless, gastroenterologists (GI) routinely miss approximately 25% of polyps during colonoscopies. These misses are highly operator dependent, influenced by the physician skills, experience, vigilance, and fatigue. Standard quality metrics, such as Withdrawal Time or Cecal Intubation Rate, have been shown to be well correlated with Adenoma Detection Rate (ADR). However, those metrics are limited in their ability to assess the quality of a specific procedure, and they do not address quality aspects related to the style or technique of the examination. In this work we design novel online and offline quality metrics, based on visual appearance quality criteria learned by an ML model in an unsupervised way. Furthermore, we evaluate the likelihood of detecting an existing polyp as a function of quality and use it to demonstrate high correlation of the proposed metric to polyp detection sensitivity. The proposed online quality metric can be used to provide real time quality feedback to the performing GI. By integrating the local metric over the withdrawal phase, we build a global, offline quality metric, which is shown to be highly correlated to the standard Polyp Per Colonoscopy (PPC) quality metric.

==> figures/clustering/bic.tex <==
\begin{figure*}[h]

\centering
\captionsetup[subfigure]{labelformat=empty,justification=centering,aboveskip=1pt,belowskip=1pt}
    \begin{tabular}[c]{c c}
    \centering
    
    \begin{subfigure}[t]{0.48\textwidth}
        \tikzset{mark options={mark size=1.25, line width=1pt}}
        \begin{tikzpicture}
            \begin{axis}[
            width=5.95cm, height=4.25cm,
            ylabel near ticks,
            xlabel near ticks,
            xlabel=\# of components,
            ylabel=BIC,
            axis lines=left,
            scaled ticks=true,
            xmin=0, xmax=8,
            legend pos=south east,
        	legend style={font=\small}
            ]
        
            \addplot[color=blue, mark=*, line width=0mm,] coordinates {
            (1, -14459543)
            (2, -20758120)
            (3, -23034443)
            (4, -26497061)
            (5, -26021402)
            (6, -24668838)
            (7, -23445566)
            (8, -22095709)
            };
            
            \addplot[color=blue,error bars/.cd, y dir=both,y explicit,]
            coordinates {
            (1, -14459543) +- (0, 0)
            (2, -20758120) +- (0, 1771078)
            (3, -23034443) +- (0, 2437098)
            (4, -26497061) +- (0, 2011839)
            (5, -26021402) +- (0, 1990580)
            (6, -24668838) +- (0, 1582427)
            (7, -23445566) +- (0, 1866341)
            (8, -22095709) +- (0, 1862011)
            };
            
            \node (mark) [draw, green, circle, minimum size = 5pt, inner sep=3pt, thick]
            at (axis cs: 4, -26497061) {};

            \end{axis}
        \end{tikzpicture}

    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.48\textwidth}
        \tikzset{mark options={mark size=1.25, line width=1pt}}
        \begin{tikzpicture}
            \begin{axis}[
            width=5.95cm, height=4.25cm,
            ylabel near ticks,
            xlabel near ticks,
            xlabel=\# of components,
            ylabel={Entropy [nat]},
            axis lines=left,
            scaled ticks=true,
            xmin=0, xmax=8,
            legend pos=south east,
        	legend style={font=\small}
            ]
        
            \addplot[color=red, mark=*, line width=0mm,] coordinates {
            (1, 0)
            (2, 0.4046387)
            (3, 0.6795597)
            (4, 0.9046586)
            (5, 1.0969184)
            (6, 1.1306816)
            (7, 1.2462864)
            (8, 1.1448100)
            };
            
            \addplot[color=red,error bars/.cd, y dir=both,y explicit,]
            coordinates {
            (1, 0) +- (0, 0)
            (2, 0.4046387) +- (0, 0.316740)
            (3, 0.6795597) +- (0, 0.249038)
            (4, 0.9046586) +- (0, 0.303143)
            (5, 1.0969184) +- (0, 0.159019)
            (6, 1.1306816) +- (0, 0.193238)
            (7, 1.2462864) +- (0, 0.170235)
            (8, 1.1448100) +- (0, 0.169997)
            };
            
            \node (mark) [draw, black, circle, minimum size = 5pt, inner sep=3pt, thick]
            at (axis cs: 5, 1.0969184) {};
        
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}
    
    \end{tabular}
\caption{\textbf{The effect of number of clusters.} For different numbers of GMM components, the BIC scores are shown on the left, and the entropy on the right.}
\label{fig:bic_ent}
\end{figure*}

==> figures/embedding/embedding-pseudo.tex <==
\begin{figure*}[h]
\begin{center}
\tikzset{mark options={mark size=0.5, line width=1pt}}
\begin{tikzpicture}
    \begin{axis}[
    % axis x line=middle,
    % axis y line=middle,
    xmin=-120, xmax=120,
    ymin=-100, ymax=100,
    legend style={font=\small},
    legend pos=south east,
    enlarge y limits=true,
    width=12cm, height=8cm,
    xlabel={$tSNE_x$},
    ylabel={$tSNE_y$},
    axis lines=left,
    clip=false
    ]

    
    \addplot[only marks, green] table [x=x, y=y, col sep=comma] {figures/embedding/data/manifold-resnetrs-50777894-noninformative.csv};
    
    \addplot[only marks, blue] table [x=x, y=y, col sep=comma] {figures/embedding/data/manifold-resnetrs-50777894-outside.csv};
    
    \addplot[only marks, cyan] table [x=x, y=y, col sep=comma] {figures/embedding/data/manifold-resnetrs-50777894-polyp.csv};
    
    \addplot[only marks, magenta] table [x=x, y=y, col sep=comma] {figures/embedding/data/manifold-resnetrs-50777894-tool.csv};
    
    \addplot[only marks, gray] table [x=x, y=y, col sep=comma] {figures/embedding/data/manifold-resnetrs-50777894-tube.csv};
    
    
    \legend{Noninformative,Outside,Polyp,Tool,Tube}
    \end{axis}
\end{tikzpicture}
\end{center}

\caption{\textbf{Pseudo labels.} .}
\label{fig:pseudo}
\end{figure*}

==> figures/global/cluster1-detected-scatter.tex <==
\begin{figure*}[h]

\pgfplotstableread[col sep = comma]{figures/global/data/manifold-500.csv}\loadedtable
\begin{center}
\tikzset{mark options={mark size=1.0, line width=1pt}}
\begin{tikzpicture}
    \begin{axis}[
    % axis x line=middle,
    % axis y line=middle,
    enlarge y limits=true,
    width=10cm, height=7cm,
    xlabel={$Q_{\text{MLP}}$ [secs]},
    ylabel={\# Polyps},
    axis lines=left,
    clip=false
    ]
    \addplot[scatter, only marks] table [x=sum_secs, y=polyp, col sep=comma] {\loadedtable};
    % \addplot [no markers] table [x=sum_1_all_secs, y={create col/linear regression={x=sum_1_all_secs, y=sum_detect_secs}}] {\loadedtable};
    \end{axis}
\end{tikzpicture}
\end{center}

\caption{\textbf{Detected correlation.} }
\end{figure*}

==> figures/global/polyp-vs-no-polyp-hist.tex <==
\begin{figure*}[h]

\pgfplotstableread[col sep = comma]{figures/global/data/sum-secs-hist-polyps-no-polyps.csv}\loadedtable
\begin{center}
\tikzset{mark options={mark size=1.5, line width=1pt}}
\begin{tikzpicture}
    \begin{axis}[
    % enlarge y limits=true,
    width=10cm, height=7cm,
    ybar,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2},
    bar width=12.0,
    xlabel={$Q_{\text{MLP}}$ [Secs]},
    ylabel={Relative frequency},
    ylabel near ticks,
    xlabel near ticks,
    scaled ticks=true,
    xmin=0, xmax=200,
    ymin=0, ymax=0.5,
    % ytick={0.05,0.1,0.15,0.2},
    ]
    \addplot [color=blue,fill] table [x=division, y=no_polyp_normed, col sep=comma] {\loadedtable};
    \addplot [color=red,fill] table [x=division, y=polyp_normed, col sep=comma] {\loadedtable};
    \legend{Polyps free, Polyps observed};
    \end{axis}
\end{tikzpicture}
\end{center}

\caption{\textbf{$Q_{\text{MLP}}$ during the withdrawal phase.} Procedures with high $Q_MLP$ values are likely to have polyps.}
\label{fig:hists}
\end{figure*}

==> figures/global/polyps-detections.tex <==
\begin{figure*}[h]

\centering
\captionsetup[subfigure]{labelformat=empty,justification=centering,aboveskip=1pt,belowskip=1pt}
    \begin{tabular}[c]{l r}
    \centering
    
    \begin{subfigure}[t]{0.5\textwidth}
        \begin{tikzpicture}
            \begin{axis}[
            enlarge y limits=true,
            width=6.25cm, height=5cm,
            xlabel={$Q_{\text{Offline}}$},
            ylabel={Detection},
            axis lines=left,
            ylabel near ticks,
            xlabel near ticks,
            scaled ticks=true,
            clip=false,
            ]
            \addplot[only marks, color=red, mark=*, mark size=1.2pt] table [x=predict, y=detect, col sep=comma] {figures/global/data/measures-global-10c_5.csv};
            \end{axis}
        
        \end{tikzpicture}

    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.5\textwidth}
        \begin{tikzpicture}
            \begin{axis}[
            enlarge y limits=true,
            width=6.25cm, height=5cm,
            xlabel={$Q_{\text{Offline}}$},
            ylabel={\# Polyps},
            axis lines=left,
            ylabel near ticks,
            xlabel near ticks,
            scaled ticks=true,
            clip=false,
            ]
            \addplot[only marks, color=blue, mark=*, mark size=1.2pt] table [x=predict, y=polyp, col sep=comma] {figures/global/data/measures-global-10c_5.csv};
            \end{axis}
        
        \end{tikzpicture}
    \end{subfigure}
    
    \end{tabular}
\caption{Analyzing the relationship between the suggested method and the absolute polyp frame detection scores (left) and the true number of polyps found in the procedure (right). As can be seen, the proposed measure is strongly correlated with the presence of polyps.}
\label{fig:buckets_and_hists}
\end{figure*}

==> figures/global/scatter-and-hists.tex <==
\begin{figure*}[h!]

\begin{center}
\tikzset{mark options={mark size=0.5, line width=3pt}}
\begin{tikzpicture}
    \begin{axis}[
    enlarge y limits=true,
    width=10cm, height=6cm,
    xlabel={$Q_{\text{Offline}}$},
    ylabel={Detection},
    axis lines=left,
    ylabel near ticks,
    xlabel near ticks,
    scaled ticks=true,
    clip=false,
    ]
    \addplot[scatter, only marks] table [x=predict, y=polyp, col sep=comma] {figures/global/data/measures-global-10c_5.csv};
    \end{axis}

\end{tikzpicture}
\end{center}
\caption{\textbf{$Q_{\text{Offline}}$ during the withdrawal phase.} Analyzing the relationship between the suggested method and absolute polyp frame detection scores in each procedure. As can be seen, the proposed  measure is strongly correlated with the presence of polyps.}
\label{fig:bic_ent}

\end{figure*}

==> figures/global/scatter-detects.tex <==
\begin{figure}
\begin{center}
% \tikzset{mark options={mark size=0.5, line width=3pt}}
\begin{tikzpicture}
    \begin{axis}[
    enlarge y limits=true,
    width=9cm, height=5cm,
    xlabel={$Q_{\text{Offline}}$},
    ylabel={Detection},
    axis lines=left,
    ylabel near ticks,
    xlabel near ticks,
    scaled ticks=true,
    clip=false,
    ]
    \addplot[only marks, color=blue, mark=*, mark size=1.2pt] table [x=predict, y=detect, col sep=comma] {figures/global/data/measures-global-10c_5.csv};
    \end{axis}

\end{tikzpicture}
\end{center}
\caption{Examining the relationship between the suggested method and absolute polyp frame detection scores in each procedure. As can be seen, the proposed  measure is strongly correlated with the presence of polyps.}
\label{fig:bic_ent}

\end{figure}

==> figures/global/scatter-polyps.tex <==
\begin{figure}

\begin{center}
% \tikzset{mark options={mark size=0.5, line width=3pt}}
\begin{tikzpicture}
    \begin{axis}[
    enlarge y limits=true,
    width=9cm, height=5cm,
    xlabel={$Q_{\text{Offline}}$},
    ylabel={\# Polyps},
    axis lines=left,
    ylabel near ticks,
    xlabel near ticks,
    scaled ticks=true,
    clip=false,
    ]
    \addplot[only marks, color=blue, mark=*, mark size=1.2pt] table [x=predict, y=polyp, col sep=comma] {figures/global/data/measures-global-10c_5.csv};
    \end{axis}

\end{tikzpicture}
\end{center}
\caption{Analyzing the relationship between the suggested method and the true number of polyps found in the procedure. As can be seen, the proposed measure is strongly correlated with the presence of polyps.}
\label{fig:sm_polyps}

\end{figure}

==> figures/samples/sm.tex <==
\begin{figure}
\centering
\captionsetup[subfigure]{labelformat=empty,justification=centering,aboveskip=1pt,belowskip=1pt}
    \begin{tabular}[c]{c c c c c c c c c c c}
    
    \centering
    
    \begin{subfigure}[t]{0.115\textwidth}
    \centering
    \caption*{Cluster}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#0}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#1}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#2}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#3}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#4}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#5}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#6}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#7}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#8}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \caption*{\#9}
    \end{subfigure}
    
    \\
    
    
    
    \begin{subfigure}[t]{0.115\textwidth}
    \centering
    \vspace{1.9cm}
    Samples
    \end{subfigure}
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c0/i63.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c0/i62.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c0/i61.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c0/i60.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c0/i59.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c0/i57.png}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c1/i48.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c1/i61.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c1/i63.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c1/i52.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c1/i51.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c1/i50.png}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c2/i51.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c2/i53.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c2/i56.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c2/i57.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c2/i60.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c2/i63.png}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c3/i56.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c3/i49.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c3/i50.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c3/i51.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c3/i55.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c4/i58.png}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c4/i51.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c4/i52.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c4/i59.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c4/i61.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c4/i57.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c4/i63.png}
    
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c5/i4.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c5/i6.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c5/i10.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c5/i30.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c5/i36.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c5/i46.png}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c6/i0.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c6/i1.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c6/i3.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c6/i4.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c6/i5.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c6/i6.png}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c7/i49.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c7/i50.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c7/i52.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c7/i55.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c7/i60.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c7/i58.png}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c8/i5.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c8/i31.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c8/i33.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c8/i38.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c8/i47.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c8/i52.png}
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{figures/samples/sm/c9/i49.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c9/i52.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c9/i54.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c9/i58.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c9/i62.png}
    \includegraphics[width=1\linewidth]{figures/samples/sm/c9/i63.png}
    \end{subfigure}
    
    \\
        %array([-1.750867  , -0.115253696, -1.1425925 , -0.79185915, -0.48000807,
        %.  0.05481249, -0.06936351, -0.17544615,  0.6582494 , -0.7127066 ],
    
    % 8 0.320556640625 7 0.140533447265625 1 0.193817138671875 5 0.067138671875 9 0.107025146484375 3 0.04205322265625 2 0.09515380859375 0 0.030731201171875 4 0.002777099609375 6 0.000213623046875
    
    
    
    \begin{subfigure}[t]{0.115\textwidth}
    \centering
    Frequency
    \end{subfigure}
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $3.07\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $19.3\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $9.51\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $4.20\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $0.27\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $6.71\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $0.02\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $14.0\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $32.0\%$
    \end{subfigure}
    
    &
    
    \begin{subfigure}[t]{0.081\textwidth}
    \centering
    $10.7\%$
    \end{subfigure}
    
    \\
    
            %array([-1.750867  , -0.115253696, -1.1425925 , -0.79185915, -0.48000807,
        %.  0.05481249, -0.06936351, -0.17544615,  0.6582494 , -0.7127066 ],
    
    
    % \begin{subfigure}[t]{0.115\textwidth}
    % \centering
    % Weight
    % \end{subfigure}
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $-1.750$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $-0.115$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $-1.142$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $-0.791$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $-0.480$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $+0.054$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $-0.069$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $-0.175$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $+0.658$
    % \end{subfigure}
    
    % &
    
    % \begin{subfigure}[t]{0.081\textwidth}
    % \centering
    % $-0.712$
    % \end{subfigure}
    
    
    \end{tabular}
\caption{Random selection of frames from each cluster along with their corresponding relative frequency. 
Clusters \#1, \#7, \#8 are more informative and their contribution is higher than other clusters.}
\label{fig:samples}
\end{figure}{}

